Mass Effects in the Higgs-Gluon Coupling: Boosted vs Off-Shell Production

In the upcoming LHC run we will be able to probe the structure ofthe loop--induced Higgs--gluon coupling through kinematics. First, we establish state-of-the-art simulations with up to two jets to next-to-leading order including top mass effects. They allow us to search for deviations from the low-energy limits in boosted Higgs production. In addition, the size of the top mass effects suggests that they should generally be included in Higgs studies at the LHC. Next, we show how off-shell Higgs production with a decay to four leptons is sensitive to the same top mass effects. We compare the potential of both methods based on the same top--Higgs Lagrangian. Finally, we comment on related model assumptions required for a Higgs width measurement.

==> Makefile <==
#-----------------------------------------------------
# This is a platform-independent Makefile to generate 
# dvi, ps and pdf files including Feynman Graphs using 
# FeynMP from the TeX source file MAIN_SRC. 
# The pdf filename is chosen via MAIN_PDF. 
#-----------------------------------------------------

MAIN_SRC = paper
MAIN_PDF = paper

ARCHFLG  = $(shell if test `uname -s` == "Darwin"; then echo "preview"; \
	else echo "ghostview"; fi) 

MAIN:
		pdflatex $(MAIN_SRC).tex
		pdflatex $(MAIN_SRC).tex

preview:
	 	$(MAKE)
		open -a Preview $(MAIN_PDF).pdf
skim:
	 	$(MAKE)
		open -a Skim $(MAIN_PDF).pdf

ghostview: 
	 	$(MAKE)
		gv -antialias $(MAIN_SRC).ps

gv:
		$(MAKE) $(ARCHFLG)

tar:
		make clean
		tar czvf $(MAIN_SRC).tar.gz *.tex *.eps Makefile

arxiv:
		make clean
		tar czvf $(MAIN_SRC).tar.gz *.tex *.eps

feyn:


clean:
		rm -f *.log *.1 *.t1 *.mp *.dvi $(MAIN_SRC).ps $(MAIN_SRC).pdf *.aux *.pdfsync *.rel
		rm -f *.toc *.lof $(MAIN_SRC).tar.gz


==> ordercite <==
#!/usr//bin/perl -w
# 
# Place this file in your bin directory.
# Make it executable (chmod +x ordercite). 
# If your copy of perl is not in /usr/bin/perl, then you will need
# to modify the first line of this file to point to it.

# Instructions on running the program can be obtained by running
# ordercite without any arguments.
#
# $Id: ordercite,v 1.6 2004/07/12 23:21:38 salam Exp $

# CHANGELOG:
# - ??/12/2003 (v3.0): wrote this to replace C++ version
# - 08/07/2004 (v3.1): added "-nochecks" option so as to generate reordered
#                      list even if there are missing citations/refs/etc. 


use strict;

(my $name= "$0") =~ s/.*\///;

if ($#ARGV < 0) {print "Usage:

> $name filename.tex [-nochecks]
".'
The program will indicate whether references are in order and whether
there are any missing references/citations. If there are no missing
references/citations but the references are in the wrong order a file
filename.tex.newref will be generated containing the reordered
references. (With the "-nochecks" option a reordered list will always 
be generated)

Note that the determination of the order and existence of
references/citations is based on the filename.aux file. This is quite
robust, but LaTeX must have been run first. 

On the other hand the reordering of the references is less robust, and
will for example break if there are strings such as "\\\\bibitem" or 
"\%[...]\bibitem" In most cases (all?) an error message will be
generated if there are signs of problems and no .tex.newref file will
be produced.
'; exit }

my $basefile='';
my $nochecks = 0;

while (my $arg = shift @ARGV) {
  if ($arg eq '-nochecks') {$nochecks = 1}
  elsif ($arg !~ /^-/) {$basefile = $arg}
  else {die "Unrecognized option $arg"}
}
if ($basefile eq '') {die "basefile not specified"}

#(my $basefile = $ARGV[0]) =~ s/\.tex$//;
$basefile =~ s/\.tex$//;
$basefile =~ s/\.aux//;
my $auxfile = $basefile.".aux";
my $texfile = $basefile.".tex";

#-- check aux file is sufficiently recent
(my @details = stat $texfile) || die "Error: problem accessing $texfile\n";
# time since it was last changed (name changes also matter)
my $textime = $details[10];
(@details = stat $auxfile)  || die "Error: problem accessing $auxfile\n";
my $auxtime = $details[10];
if ($auxtime <= $textime) {
  die "Error: $auxfile should be more recent than $texfile, but is not. Run LaTeX!\n"}


my %references = ();
my @references = ();

my %citations = ();
my @citations = ();

my $problems = 0;
my $mismatches = 0;
my $key;

# read in aux file
open(AUX , "< $auxfile") || die "Could not open $auxfile";
while (my $line=<AUX>) {
  chomp($line);
  if ($line =~ /^\\citation/) {
    $line =~ s/.*{(.*)}/$1/;
    my @keys = split(',', $line);
    foreach my $key (@keys) {
      if (!exists($citations{$key})) {
	push @citations, $key;
	$citations{$key} = 1;
	#print "$key\n";
      }
    }
  }
  if ($line =~ /^\\bibcite/) {
    # add extra bracket at end so as not to confuse emacs bracket counting!
    $line =~ s/[^{]*{(.*)}[^}]*/$1/;
    (my $key, my $numb) = split('}{', $line);
    if (exists($references{$key})) {
      print STDERR "WARNING: $key appeared more than once in references\n";
      $problems += 1;
    }
    else{
      push @references, $key;
      $references{$key} = $numb;
      if ($numb ne $#references+1) {
	print "WARNING: problem in numbering of references for $key";
	$problems += 1;
      } 
    }
  }
}

#======= summarise status of aux file ==================================
my %absentcitations=();
my %absentreferences=();
foreach $key (keys %citations) {
    if (!exists $references{$key}) {$absentreferences{$key}=1}}
foreach $key (keys %references) {
  if (!exists $citations{$key}) {$absentcitations{$key}=1}}

my $format = "%5u%32s%32s%6s";
(my $formattit = $format) =~ s/u/s/;
my $separator="--------------------------------------------------------------------------\n";
my $summary='';
$summary .= sprintf ($formattit,"","Citation","Reference","")."\n";
$summary .= $separator;
my $maxindex = max($#references,$#citations);
for (my $index=0; $index <= $maxindex; $index++) {
  my $ne; my $citation; my $reference;
  if ($index > $#citations) {$citation = ''} else 
    {$citation = $citations[$index]}
  if ($index > $#references) {$reference = ''} else 
    {$reference = $references[$index]}
  if ($citation eq $reference){$ne = ''}else{ $ne = '*'}
  $summary .= sprintf("%5u%32s%32s%5s",$index+1,$citation,$reference,$ne)."\n";
  if ($ne ne '') {$mismatches += 1};
}
$summary .= $separator;

if ($mismatches == 0) {print "All references and citations match and appear in correct order!\n"; exit}

print $summary;

# check to see if anything is missing
my @rlist = (keys %absentreferences);
if ($#rlist >= 0) {
  print "The following references were cited but not present in bibliography:\n",
    join("\n",@rlist),"\n",$separator;
}
my @clist = (keys %absentcitations);
if ($#clist >= 0) {
  print "The following references were present in bibliography but not cited:\n",
    join("\n",@clist),"\n",$separator;
}

#======= Reorder citations? ==================================
if ((($#rlist >= 0 || $#clist >= 0 || $mismatches == 0) && (!$nochecks)) || $problems > 0) {
  print "Will not attempt to create a reordered citation list!\n";
  exit;
}
open (TEX, "<$texfile") || die "Could not open $texfile.\n";
my $collecting = 0;
my $current='';
my $next = '';
my $index=-1;
my $result = '';
my $seenblankline=0;

#-- first split lines with a bibitem; not very elegant, but sometimes useful
#   NB: things such as \% and \\bibitem are not properly dealt with!
#   (not very effecient? Better to do on just restricted part of file)
my @lines = ();
while (my $line = <TEX>){
  if ($line !~ /\\bibitem/) {push @lines, $line;}
  else {
    my $extractor = qr/^([\s]*[^%\s]+[^%]*)(\\bibitem.*)/;
    my @lcllist = ();
    while ($line =~ /$extractor/) {
      (my $lastbib = $line) =~ s/$extractor/$2/;
      push @lcllist, $lastbib;
      $line =~ s/$extractor/$1/;
    }
    push @lines, $line, reverse(@lcllist);
  }
}
# handy for debugging...
#print join('',@lines)."\n";
close(TEX);


for my $line (@lines){
  if ($line =~ /^[^%]*\\begin{thebibliography}/) {
    die "Found \\begin{thebibliography} inside bibliography" unless !$collecting; 
    $collecting = 1;
    $result .= $line;
   next;
  }
  if ($line =~ /^[^%]*\\end{thebibliography}/) {
    die "Found \\end{thebibliography} outside bibliography" unless $collecting; 
    $references{$references[$index]} = $current;

    # make sure no references have gone missing...
    if ($index != $#references) {
      die 
       "Error: number of bibitems found (".($index+1).") does not correspond 
       to expected number of references (".($#references+1).").\n"
    }

    # now collect all references in the right order
    for ($index=0; $index <= $#citations; $index++){
      if (!exists $references{$citations[$index]}) {
	print STDERR "Could not find reference ".$citations[$index]."\n";
      } else { $result .= $references{$citations[$index]}}
    }
    # put on any "post matter"
    $result .= $next;
    # finish off the bibliography
    $result .= $line;

    # now put commented version of references that were not cited
    $result .= "\n";
    foreach my $absentee (@clist) {
      (my $absref = $references{$absentee}) =~ s/^/%% /mg;
      $result .= $absref;
    }
    $result .= "\n";

    last;
  }
  next unless $collecting;

  if ($line =~ /^[\s]*\\bibitem/) {
    # tidy up last citation
    if ($index >=0) {
      $references{$references[$index]} = $current
    } else {$result .= $current}

    $seenblankline = 0;
    $index+=1;
    $current = $next.$line;
    $next = '';
    ($key = $line) =~ s/.*bibitem{(.+?)}.*/$1/;
    chomp ($key);
    if ($references[$index] ne $key) {
      die  "Error: Reference ".($index+1)." (".$references[$index].
	") does not match with expected key $key.\n";
    }
    next;
  } 
  
  # now arrange so that any comment after a blank line goes
  # into the next citation, UNLESS it is followed by non-commented
  $seenblankline = ($seenblankline || ($line =~ /^[\s]*$/));
  if ($seenblankline && $line =~ /^[\s]*[^%\s]/) {
    $seenblankline =0; $current.=$next; $next = ''
  }
  if ($seenblankline) {$next .= $line} else {$current .= $line}
}
print "Creating file $texfile.newref with reordered references (use with caution!)\n";
open (REFOUT, "> $texfile.newref");
print REFOUT $result;

#======================================================================
# yeah, so it's f90 like, etc...
sub max {
  (my $a, $b) = @_;
  if ($a > $b) {return $a} else {return $b}
} 

